Leveraging Knowledge Bases And Parallel Annotations For Music Genre Translation

Prevalent efforts have been put in automatically inferring genres of musical items. Yet, the propose solutions often rely on simplifications and fail to address the diversity and subjectivity of music genres. Accounting for these has, though, many benefits for aligning knowledge sources, integrating data and enriching musical items with tags. Here, we choose a new angle for the genre study by seeking to predict what would be the genres of musical items in a target tag system, knowing the genres assigned to them within source tag systems. We call this a translation task and identify three cases: 1) no common annotated corpus between source and target tag systems exists, 2) such a large corpus exists, 3) only few common annotations exist. We propose the related solutions: a knowledge-based translation modeled as taxonomy mapping, a statistical translation modeled with maximum likelihood logistic regression; a hybrid translation modeled with maximum a posteriori logistic regression with priors given by the knowledge-based translation. During evaluation, the solutions fit well the identified cases and the hybrid translation is systematically the most effective w.r.t. multilabel classification metrics. This is a first attempt to unify genre tag systems by leveraging both representation and interpretation diversity.

==> sources/algs_steps.tex <==
\iffalse
\begin{algorithm}
\caption{Implementing $g$ DBpedia mapping function.}
\label{alg:dbpmap}
\begin{algorithmic}[1]
\Require 
\State $D$: input genre definition, set of tags and relations
\State $B$: DBpedia genre definition, set of tags and relations
\Ensure
\State $\Theta$: the translation table
\Function{DBpediaMapping}{$D$, $B$}
\State $unmapGs \gets []$ \Comment{List of unmapped genres}
\State init $\Theta$ matrix with \Call{NormGenres}{$B$} as columns
\ForEach  {$sg \in$ \Call{NormGenres}{$D$}}
	\State  $coreGs \gets$  \Call{DBCoreGenres}{$sg$, $B$, $D$}
	\Comment{Dictionary with the most related DBpedia genres and their relateness scores}
    \If{$length(coreGs)=0$}
    	\State add $sg$ to $unmapGs$ \Comment{Handle it after}
    \Else 
     	\State  $neighGs \gets$  \Call{NeighGenres}{$coreGs$,$B$} \Comment{Dictionary with the neighbour genres of $coreGs$ and their relatedness scores}
     	\State update $\Theta[sg]$ with $coreGs$ and $neighGs$
    \EndIf
\EndFor 
\ForEach  {$s \in unmapGs$}
    \State  $rowVals \gets$  \Call{AvgRelatedGenres}{$s$,$D$,$\Theta$} \\ \Comment{average over subgenre and parent genres of $sg$ in $\Theta$}
    \State $\Theta[s] \gets rowVals$
\EndFor
\State \Return $\Theta$
\EndFunction
\end{algorithmic}
\end{algorithm}


\begin{algorithm}
\caption{Identifying the most related DBpedia genres.}
\label{alg:dbpmap2}
\begin{algorithmic}[1]
\Require 
\State $sg$: the source genre
\State $D$: input genre definition, set of tags and relations
\State $B$: DBpedia genre definition, set of tags and relations
\Ensure
\State a dictionary with the most related DBPedia genres as keys and their relatedness scores as values
\Function{DBCoreGenres}{$sg$,$B$,$D$}
\If{$sg$ in $B$}
    \State $aliasGs \gets$ \Call{DBAliases}{$sg$,$B$}  \Comment{Return its DBpedia aliases, including $sg$}
    \State return dict($aliasGs$, 1) \Comment{Return a dictionary with keys $aliasGs$ and all values set to 1}
\EndIf
\State
\State $parentGs \gets$ \Call{NormParentGenres}{s, $D$} \Comment{Parent genres in the input genre definition}
\ForEach  {$pg \in parentGs$}
    \State $compG \gets$ \Call{NormComposedGenre}{$pg$, $sg$} \Comment{Normalized label, formed by concatenating $pg$ to $sg$}
    \If{$compG$ in $B$}
    \State $aliasGs \gets$ \Call{DBAliases}{$compG$,$B$} 
    \State return dict($aliasGs$, 1)
    \EndIf
\EndFor
\State
\If{\Call{GraphType}{$sg$}=Genre/Concept}
    \State $dbGs \gets$ \Call{DBGenresContain}{$sg$} \Comment{DBpedia genres containing the word $sg$}
    \State $graph \gets$ \Call{DBSubgraph}{$dbGs$} \Comment{DBpedia directed subgraph with these nodes only}
    \State $coreGs \gets$ argmax(\Call{InDegrees}{$graph$}) \Comment{DBpedia genres with maximum in-degree value}
\EndIf
\State
\If{\Call{GraphType}{$sg$}=ComposedGenre}
    \State $dbGs \gets$ \Call{DBGenresShareWords}{$sg$} \Comment{DBpedia genres and number of words shared with $sg$}
    \State $coreGs \gets$ arxmax($dbGs$) \Comment{DBpedia genres sharing the maximum number of concepts with $sg$}
    \State $coreGs \gets$ \Call{WithGenreConcepts}{$coreGs$} \Comment{Select genres which contain genre/concepts among the shared words if any; if not $coreGs$ stay unchanged}
    \State $aliasGs \gets$ \Call{DBAliases}{$coreGs$,$B$} 
\EndIf
\State return dict($coreGs$, 1/length($coreGs$))
\EndFunction
\end{algorithmic}
\end{algorithm}

Steps of the algorithm
\begin{itemize}

    \item For each normalized source genre, identify the most related genres from the DBpedia tags
    \item Then compute the relatedness scores for the neighbours of these most related genres. The score is computed by taking as reference the score of the original genre and divide it by 2. So it is twice less important in the ranks. 
    Only subgenre and origin relations are considered; derivative relations did not lead to better results experimentally.
    \item if no most related genres are identified, keep track of these genres not mapped. Then, go through the genres not mapped and find out what are the related genres of each genre, in the source taxonomy (could be parent genre or subgenre). Compute its translation vectors by averaging the translation vectors of its related genres.
\end{itemize}

How the mapping of a genre on DBpedia genres takes place. There are multiple situations:
\begin{itemize}
    \item the normalized genre is directly found among the DBpedia normalized genres. Then, the genre and its aliases get a score of 1
    \item then maybe if the label does not exist directly in DBpedia, try to see if disambiguating the label with its supra-genre works. Specifically try to see if normalized concatenation of the label and its supragenre's label is found in DBpedia normalized tags. If yes process as above
    \item If not, treat each tag depending on the type. if it is a concept/genre it's likely that is one of the main genres. If yes find out all dbpedia genres which have the normalized form containing this word. Get the subgraph composed of these nodes only, compute the in-centrality and sort them descendingly. From this list retrieve the top tags (all tags which have the in-centrality equal to max). The score is divided between the options (1/ number of candidates);
    \item if the tag is a composed genre the approach is different. Find out all the dbpedia genres that share at least one word with this genre. First try to see if among the candidates it's a genre that contains all words of the composed genre and if yes process it.
    If not, find out the genres that contain the maximum number of concepts and also constrain that one concept among the maximum number of concept shared is a genre/concept. If candidates are found in this way return them, otherwise return all the dbpedia genres (with a low score) 
\end{itemize}
\fi

==> sources/literature.tex <==
%All related works aim at assessing the relevance of target concepts for a given source concept.
%In a supervised setup, \cite{Spohr2011} represent each source concept through a list of string- and structure-related features derived only from taxonomies.
%\cite{Papadimitriou} achieve the goal by using a parallel corpus annotated with both source and target taxonomies; the item title, attributes and descriptions are features.
%Some other works use instead unsupervised setups \cite{AANEN2015,Ponzetto:2009}.
%We acknowledge the utility of both setups but for different objectives. 
%We implement unsupervised taxonomy mapping when no parallel corpus is available and supervised otherwise.
%There are also significant differences compared to the related works.
%First, we consider also the case when multiple source taxonomies have to be aligned together on a target taxonomy.
%Second, in the supervised approach, we use as item features just the set of tags comings from the input taxonomies.
%Third, we combine the two in a Bayesian approach, using the alignment of taxonomies as a prior for training classifiers when annotations are available.
%Fourth, more specific differences regarding the unsupervised taxonomy mapping are discussed further.


%supervised: machine learning with a corpus containing for each concept 20 similarity vectors corresponding to exact, close and bad matches \cite{Spohr2011}
%\cite{Papadimitriou}: 
%supervised machine learning, uses a common annotated dataset, they use the text available on items which contain the title, attributes and descriptions; similar to us it's a multi-label classification but we exploit instead the annotations coming from multiple sources. 
%The final solution is an optimization problem on top of the baseline: corrects the scores predicted by the baseline by taking into consideration the structure
%\cite{Ponzetto:2009} 
%disambiguate each wikipedia category on a wordnet synset; 
%generated a restructured version of wikipedia by considering the relations between concepts in wordnet
%\cite{Swoboda:2016} evolve a specific taxonomy in another one with categories adopted from a general, large taxonomy. 
%The problem is modeled differently, instead of aligning is to find the most relevant categories from a target that should be added to a source.
%The relevance is computed as cosine similarity between the word2vec vectors for categories.
%\cite{Prytkova:2015} 
%one to one disambiguation using wikipedia as an intermediate. 
%the similarity of each category of source and target taxonomies to each wikipedia category is measured. 
%then the candidates are generated from all pairs that share labels. 
%the solution is modeled using combinatorial optimization (integer linear programming and quadratic programming).
%\cite{Wu:2016:CTA} 
%focused on how to measure the relevance between one source category and one target category. 
%String similarity leads to poor results, but vector similarity appear as a good alternative that however needs more text. 
%Step 1: uses babel net to check if 2 categories share synonyms; 
%to get more text for each category in different context search by parent + concept. 
%step 3 translate the text in target and compute topic vectors. 
%No structural info used. we also do a candidate selection like in this work.
%Notes literature:
%\cite{Hennequin2018}
%-genre representation: 
%embeddings of genre tags are build differently. First a classifier will predict the genre from an audio excerpt 
%\textbf{Music Genre Representation}
%\label{sec:manualGenreAnnotation}
%\begin{itemize}
%    \item Expert annotations
%    \item Social tags and folksonomies
%    \item Challenges with perception, cultural factors
%\end{itemize}
%mention that the only other work using node embedding from ontologies is Doremus and is used for the medium of performance
 % \cite{Craft}
% "Ground truth is an artefact of an individual’s response to music, not an artefact of the audio itself" "Whilst it may be useful to have a genre labelling of a dataset that is entirely unambiguous, it is also unrealistic: a practical categorisation system needs to be able to deal with all tracks, not just unambiguous data."
 


%the difference from our work is :
%"taking some properties of the track as input, like audio lyrics and such and trying to predict a tag" while we take taxonomies and predict tags from another taxonomy
%"usually when you talk about genre classification there is only one genre ontology which is agreed upon and serves as ground truth. Then the goal is to use accessory data (which are not genre) to predict the genre."

%Talk about using priors, incorporating prior knowledge

